Harnessing Mixed Offline Reinforcement Learning Datasets via Trajectory Weighting

Most offline reinforcement learning (RL) algorithms return a target policy maximizing a trade-off between (1) the expected performance gain over the behavior policy that collected the dataset, and (2) the risk stemming from the out-of-distribution-ness of the induced state-action occupancy. It follows that the performance of the target policy is strongly related to the performance of the behavior policy and, thus, the trajectory return distribution of the dataset. We show that in mixed datasets consisting of mostly low-return trajectories and minor high-return trajectories, state-of-the-art offline RL algorithms are overly restrained by low-return trajectories and fail to exploit high-performing trajectories to the fullest. To overcome this issue, we show that, in deterministic MDPs with stochastic initial states, the dataset sampling can be re-weighted to induce an artificial dataset whose behavior policy has a higher return. This re-weighted sampling strategy may be combined with any offline RL algorithm. We further analyze that the opportunity for performance improvement over the behavior policy correlates with the positive-sided variance of the returns of the trajectories in the dataset. We empirically show that while CQL, IQL, and TD3+BC achieve only a part of this potential policy improvement, these same algorithms combined with our reweighted sampling strategy fully exploit the dataset. Furthermore, we empirically demonstrate that, despite its theoretical limitation, the approach may still be efficient in stochastic environments. The code is available at https://github.com/Improbable-AI/harness-offline-rl.

==> iclr2022/backup_table.tex <==


% \begin{table}
% \centering
% \scriptsize
% \begin{tabular}{cl|llll|lll|llll}
% \multicolumn{1}{l}{}              &                       & \multicolumn{4}{c|}{Uniform} & \multicolumn{3}{c|}{Aw} & \multicolumn{4}{c}{Rw}       \\
% \multicolumn{1}{l}{Ratio}         & Dataset               & IQL  & CQL  & TD3+BC & BC    & IQL  & CQL  & TD3+BC    & IQL  & CQL  & TD3+BC & BC    \\ 
% \hline
% \multirow{8}{*}{0.01}             & ant-expert-v2         & 0.25 & 0.08 & 0.26   & 0.30  & 0.54 & 0.80 & 0.19      & 0.54 & 0.74 & 0.20   & 0.31  \\
%                                   & ant-medium-v2         & 0.39 & 0.14 & 0.32   & 0.31  & 0.82 & 0.79 & 0.51      & 0.82 & 0.80 & 0.42   & 0.35  \\
%                                   & halfcheetah-expert-v2 & 0.03 & 0.25 & 0.06   & 0.02  & 0.03 & 0.39 & 0.04      & 0.04 & 0.38 & 0.04   & 0.03  \\
%                                   & halfcheetah-medium-v2 & 0.21 & 0.40 & 0.16   & 0.02  & 0.16 & 0.41 & 0.20      & 0.20 & 0.42 & 0.19   & 0.03  \\
%                                   & hopper-expert-v2      & 0.12 & 0.09 & 0.19   & 0.04  & 0.55 & 0.84 & 0.57      & 0.50 & 0.52 & 0.62   & 0.16  \\
%                                   & hopper-medium-v2      & 0.53 & 0.30 & 0.30   & 0.04  & 0.39 & 0.61 & 0.52      & 0.50 & 0.58 & 0.56   & 0.34  \\
%                                   & walker2d-expert-v2    & 0.12 & 0.03 & 0.07   & 0.01  & 0.29 & 0.57 & 0.68      & 0.28 & 0.54 & 0.88   & 0.02  \\
%                                   & walker2d-medium-v2    & 0.36 & 0.03 & 0.13   & 0.01  & 0.46 & 0.46 & 0.12      & 0.48 & 0.48 & 0.16   & 0.05  \\ 
% \hline
% \multirow{8}{*}{0.05}             & ant-expert-v2         & 0.60 & 0.15 & 0.36   & 0.31  & 1.16 & 1.06 & 0.52      & 1.19 & 1.06 & 0.46   & 1.08  \\
%                                   & ant-medium-v2         & 0.73 & 0.50 & 0.62   & 0.31  & 0.88 & 0.88 & 0.99      & 0.91 & 0.93 & 0.81   & 0.86  \\
%                                   & halfcheetah-expert-v2 & 0.04 & 0.30 & 0.11   & 0.02  & 0.66 & 0.67 & 0.64      & 0.71 & 0.66 & 0.60   & 0.11  \\
%                                   & halfcheetah-medium-v2 & 0.33 & 0.47 & 0.24   & 0.02  & 0.43 & 0.47 & 0.47      & 0.41 & 0.47 & 0.47   & 0.36  \\
%                                   & hopper-expert-v2      & 0.12 & 0.10 & 0.46   & 0.04  & 1.02 & 0.99 & 0.98      & 0.87 & 0.99 & 0.87   & 0.87  \\
%                                   & hopper-medium-v2      & 0.49 & 0.43 & 0.42   & 0.05  & 0.53 & 0.65 & 0.53      & 0.56 & 0.68 & 0.54   & 0.49  \\
%                                   & walker2d-expert-v2    & 0.25 & 0.03 & 0.16   & 0.01  & 1.08 & 1.06 & 0.55      & 1.08 & 1.02 & 0.88   & 1.01  \\
%                                   & walker2d-medium-v2    & 0.58 & 0.04 & 0.05   & 0.02  & 0.58 & 0.76 & 0.79      & 0.61 & 0.75 & 0.78   & 0.56  \\ 
% \hline
% \multirow{8}{*}{0.1}              & ant-expert-v2         & 0.74 & 0.21 & 0.50   & 0.34  & 1.18 & 1.11 & 0.53      & 1.23 & 1.16 & 0.46   & 1.19  \\
%                                   & ant-medium-v2         & 0.79 & 0.57 & 0.60   & 0.45  & 0.87 & 0.91 & 1.07      & 0.90 & 0.96 & 1.14   & 0.91  \\
%                                   & halfcheetah-expert-v2 & 0.08 & 0.29 & 0.31   & 0.02  & 0.85 & 0.76 & 0.80      & 0.89 & 0.76 & 0.81   & 0.76  \\
%                                   & halfcheetah-medium-v2 & 0.40 & 0.48 & 0.43   & 0.02  & 0.45 & 0.48 & 0.48      & 0.45 & 0.48 & 0.48   & 0.42  \\
%                                   & hopper-expert-v2      & 0.18 & 0.14 & 0.65   & 0.05  & 1.00 & 1.08 & 1.02      & 1.01 & 1.03 & 1.07   & 1.05  \\
%                                   & hopper-medium-v2      & 0.46 & 0.62 & 0.23   & 0.05  & 0.55 & 0.68 & 0.57      & 0.60 & 0.71 & 0.56   & 0.57  \\
%                                   & walker2d-expert-v2    & 0.66 & 0.01 & 0.08   & 0.03  & 1.09 & 1.02 & 1.10      & 1.08 & 1.09 & 1.11   & 1.06  \\
%                                   & walker2d-medium-v2    & 0.65 & 0.24 & 0.05   & 0.06  & 0.67 & 0.79 & 0.76      & 0.64 & 0.79 & 0.62   & 0.62  \\ 
% \hline
% \multirow{8}{*}{0.5}              & ant-expert-v2         & 1.07 & 0.83 & 0.51   & 0.44  & 1.21 & 1.26 & 0.48      & 1.21 & 0.53 & 0.52   & 1.21  \\
%                                   & ant-medium-v2         & 0.91 & 0.82 & 0.92   & 0.73  & 0.92 & 0.97 & 1.11      & 0.94 & 0.94 & 1.06   & 0.89  \\
%                                   & halfcheetah-expert-v2 & 0.50 & 0.57 & 0.80   & 0.80  & 0.91 & 0.80 & 0.94      & 0.94 & 0.86 & 0.95   & 0.92  \\
%                                   & halfcheetah-medium-v2 & 0.45 & 0.49 & 0.48   & 0.10  & 0.47 & 0.49 & 0.48      & 0.47 & 0.49 & 0.48   & 0.42  \\
%                                   & hopper-expert-v2      & 0.50 & 0.82 & 0.97   & 0.04  & 1.06 & 1.03 & 1.12      & 1.07 & 1.04 & 1.10   & 1.10  \\
%                                   & hopper-medium-v2      & 0.56 & 0.73 & 0.46   & 0.03  & 0.54 & 0.63 & 0.62      & 0.52 & 0.38 & 0.61   & 0.57  \\
%                                   & walker2d-expert-v2    & 1.08 & 0.24 & 0.09   & 0.01  & 1.09 & 1.09 & 1.10      & 1.09 & 1.08 & 1.10   & 1.08  \\
%                                   & walker2d-medium-v2    & 0.67 & 0.81 & 0.07   & 0.10  & 0.63 & 0.82 & 0.80      & 0.63 & 0.83 & 0.81   & 0.72  \\ 
% \hline
% \multirow{8}{*}{1}                & ant-expert-v2         & 1.13 & 1.21 & 0.50   & 1.25  & 1.25 & 1.27 & 0.96      & 1.26 & 1.27 & 1.01   & 1.24  \\
%                                   & ant-medium-v2         & 0.99 & 0.98 & 1.20   & 0.86  & 0.97 & 0.95 & 1.16      & 0.98 & 0.97 & 1.16   & 0.88  \\
%                                   & halfcheetah-expert-v2 & 0.93 & 0.79 & 0.95   & 0.92  & 0.94 & 0.89 & 0.97      & 0.93 & 0.88 & 0.96   & 0.92  \\
%                                   & halfcheetah-medium-v2 & 0.47 & 0.49 & 0.48   & 0.43  & 0.47 & 0.49 & 0.48      & 0.47 & 0.49 & 0.48   & 0.42  \\
%                                   & hopper-expert-v2      & 0.95 & 1.05 & 1.11   & 1.09  & 1.00 & 1.05 & 1.04      & 0.96 & 1.03 & 1.10   & 1.11  \\
%                                   & hopper-medium-v2      & 0.55 & 0.74 & 0.56   & 0.52  & 0.57 & 0.71 & 0.61      & 0.57 & 0.73 & 0.62   & 0.54  \\
%                                   & walker2d-expert-v2    & 1.09 & 1.09 & 1.10   & 1.08  & 1.09 & 1.09 & 1.10      & 1.09 & 1.09 & 1.10   & 1.08  \\
%                                   & walker2d-medium-v2    & 0.75 & 0.83 & 0.82   & 0.64  & 0.69 & 0.83 & 0.80      & 0.66 & 0.82 & 0.81   & 0.71  \\ 
% \hline
% \multicolumn{1}{l}{Average score} &                       & 0.54 & 0.46 & 0.45   & 0.29  & 0.75 & 0.82 & 0.71      & 0.76 & 0.79 & 0.71   & 0.68  \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
%     \centering
%     \scriptsize
%     \begin{tabular}{llllllllllll}
%     \toprule
%           &                    & \multicolumn{6}{l}{BC} & \multicolumn{4}{l}{IQL} \\
%           &                    &           Rw (0.1) &           Uniform &               50\% &               30\% &              10\% &               1\% &           Aw (0.1) &           Aw (0.5) &           Rw (0.1) &   Uniform \\
%     Ratio & Dataset &                    &                   &                    &                    &                   &                   &                    &                    &                    &           \\
%     \midrule\hline
%     1\% & ant-expert-v2 &    \textbf{996.67} &   \textbf{940.69} &             287.30 &              65.32 &            -87.20 &           -200.58 &   \textbf{1850.63} &    \textbf{749.71} &   \textbf{1952.14} &    732.04 \\
%           & ant-medium-v2 &            1032.27 &            991.18 &             288.80 &              84.93 &            -82.78 &            -93.28 &   \textbf{3157.00} &            1238.62 &   \textbf{3097.75} &   1266.69 \\
%           & halfcheetah-expert-v2 &              20.27 &             -0.54 &             -46.40 &             -48.53 &           -107.26 &           -160.31 &    \textbf{184.53} &              24.79 &    \textbf{197.61} &    170.65 \\
%           & halfcheetah-medium-v2 &               8.23 &             -0.49 &              -0.55 &              -9.68 &            -95.59 &  \textbf{3617.65} &             913.16 &            1805.00 &   \textbf{2721.43} &   2696.51 \\
%           & hopper-expert-v2 &    \textbf{398.58} &            106.26 &             107.68 &             122.96 &             86.74 &            129.37 &   \textbf{1724.45} &    \textbf{414.66} &   \textbf{1827.65} &    348.58 \\
%           & hopper-medium-v2 &            1075.92 &            103.57 &              74.03 &             106.94 &            109.29 &            184.46 &            1616.28 &            1705.70 &            1653.51 &   1793.36 \\
%           & walker2d-expert-v2 &              82.13 &             48.30 &              31.79 &              39.61 &             44.22 &             25.51 &   \textbf{1369.49} &   \textbf{1032.59} &   \textbf{1230.69} &    517.29 \\
%           & walker2d-medium-v2 &             252.19 &             40.75 &              69.68 &              46.72 &             55.29 &             21.86 &   \textbf{2030.22} &   \textbf{2608.85} &   \textbf{2237.31} &   1624.89 \\\hline
%     5\% & ant-expert-v2 &   \textbf{4308.10} &            901.20 &             475.28 &               9.05 &           -160.98 &  \textbf{3989.67} &   \textbf{4615.38} &   \textbf{2356.30} &   \textbf{4665.57} &   2289.15 \\
%           & ant-medium-v2 &   \textbf{3303.90} &           1083.49 &             980.87 &             578.13 &             17.37 &  \textbf{3233.14} &   \textbf{3325.01} &   \textbf{3070.10} &   \textbf{3507.05} &   2824.69 \\
%           & halfcheetah-expert-v2 &   \textbf{1068.83} &             -3.81 &              -6.23 &             -33.03 &            -83.96 &           -340.79 &   \textbf{8020.04} &    \textbf{837.78} &   \textbf{8428.29} &    205.80 \\
%           & halfcheetah-medium-v2 &   \textbf{4412.19} &             -0.23 &               0.97 &             -12.25 &           1680.01 &           3505.21 &   \textbf{5012.57} &   \textbf{4426.87} &   \textbf{5078.91} &   3740.70 \\
%           & hopper-expert-v2 &   \textbf{3052.10} &             95.26 &              78.00 &             112.30 &            121.52 &   \textbf{534.57} &   \textbf{3393.28} &    \textbf{822.21} &   \textbf{2867.08} &    358.74 \\
%           & hopper-medium-v2 &            1597.58 &            138.75 &             107.42 &             125.84 &            418.38 &           1119.49 &            1601.85 &   \textbf{1660.10} &   \textbf{1756.02} &   1629.24 \\
%           & walker2d-expert-v2 &   \textbf{4695.65} &             39.22 &              36.79 &             126.92 &             56.91 &             32.71 &   \textbf{4976.50} &   \textbf{4592.57} &   \textbf{4996.24} &   1024.00 \\
%           & walker2d-medium-v2 &            2524.21 &             49.45 &             300.95 &             432.81 &            550.15 &            311.38 &   \textbf{2774.29} &            2684.90 &   \textbf{2810.30} &   2740.49 \\\hline
%     10\% & ant-expert-v2 &   \textbf{4708.27} &           1173.77 &             821.33 &             501.23 &            388.89 &  \textbf{4299.76} &   \textbf{4577.81} &   \textbf{3218.42} &   \textbf{4984.43} &   2875.40 \\
%           & ant-medium-v2 &   \textbf{3503.61} &           1639.13 &            2006.69 &            1279.31 &            856.44 &  \textbf{3313.79} &   \textbf{3262.02} &   \textbf{3213.05} &   \textbf{3471.22} &   2983.07 \\
%           & halfcheetah-expert-v2 &   \textbf{9162.78} &             -0.27 &              25.51 &    \textbf{631.20} &  \textbf{9596.41} &           -386.74 &  \textbf{10453.38} &   \textbf{3665.12} &  \textbf{10748.27} &    630.51 \\
%           & halfcheetah-medium-v2 &   \textbf{4912.14} &             -0.32 &               9.48 &              34.62 &  \textbf{4938.14} &           3223.80 &   \textbf{5246.20} &   \textbf{4978.90} &   \textbf{5339.99} &   4757.04 \\
%           & hopper-expert-v2 &   \textbf{3469.06} &            125.23 &              97.55 &             110.41 &            115.52 &  \textbf{1533.71} &   \textbf{3152.03} &   \textbf{1358.55} &   \textbf{3163.33} &    561.14 \\
%           & hopper-medium-v2 &   \textbf{1764.16} &            128.41 &             138.60 &             198.93 &            726.16 &  \textbf{1568.68} &   \textbf{1710.98} &   \textbf{1850.82} &   \textbf{1916.48} &   1483.04 \\
%           & walker2d-expert-v2 &   \textbf{4837.73} &             59.62 &              43.61 &             219.50 &             62.26 &            198.37 &   \textbf{4992.20} &   \textbf{5004.55} &   \textbf{4967.40} &   3062.34 \\
%           & walker2d-medium-v2 &            2843.62 &             52.90 &             710.33 &             600.28 &           1573.35 &           1490.45 &            3029.89 &   \textbf{3086.25} &            2903.08 &   3031.51 \\\hline
%     50\% & ant-expert-v2 &   \textbf{4782.32} &           1345.27 &            3388.32 &            3989.62 &  \textbf{5075.29} &           2972.03 &   \textbf{4779.43} &   \textbf{4666.77} &   \textbf{4910.98} &   4257.78 \\
%           & ant-medium-v2 &            3444.83 &           2950.28 &            3268.52 &            3419.29 &           3440.69 &           3063.42 &            3598.36 &            3563.90 &            3657.98 &   3671.40 \\
%           & halfcheetah-expert-v2 &  \textbf{11157.25} &  \textbf{9617.41} &  \textbf{11166.22} &  \textbf{10988.80} &           3771.37 &           -258.94 &  \textbf{10973.70} &  \textbf{10049.94} &  \textbf{11356.49} &   5716.92 \\
%           & halfcheetah-medium-v2 &            5007.50 &           1005.69 &            4863.68 &            5003.40 &           4818.18 &           3317.28 &   \textbf{5513.02} &   \textbf{5417.26} &   \textbf{5558.49} &   5316.48 \\
%           & hopper-expert-v2 &   \textbf{3569.13} &            103.60 &             145.12 &             229.66 &  \textbf{2786.99} &  \textbf{3593.61} &   \textbf{3485.90} &   \textbf{2219.13} &   \textbf{3523.62} &   1686.31 \\
%           & hopper-medium-v2 &   \textbf{1827.57} &             83.11 &             431.93 &            1194.74 &           1627.71 &  \textbf{1870.53} &            1785.05 &   \textbf{1873.90} &            1652.75 &   1821.67 \\
%           & walker2d-expert-v2 &            4970.90 &             53.99 &             216.68 &             262.58 &           1249.00 &           4985.93 &            5000.62 &            4999.96 &            5000.71 &   5004.56 \\
%           & walker2d-medium-v2 &   \textbf{3302.46} &            174.13 &            3063.65 &            2261.91 &           2553.41 &  \textbf{3382.94} &            2843.68 &   \textbf{3236.77} &            2916.00 &   3067.82 \\\hline
%     100\% & ant-expert-v2 &   \textbf{4783.87} &  \textbf{4806.57} &   \textbf{4994.22} &   \textbf{4907.91} &  \textbf{4856.83} &           -288.02 &   \textbf{5020.45} &   \textbf{4748.59} &   \textbf{4919.10} &   4486.76 \\
%           & ant-medium-v2 &            3502.41 &           3463.50 &            3565.71 &            3450.97 &           3525.09 &            419.27 &            3751.72 &            3593.66 &            3814.71 &   3851.65 \\
%           & halfcheetah-expert-v2 &           11148.84 &          11129.46 &           11080.56 &           11046.57 &           8287.45 &           -202.08 &  \textbf{11375.47} &  \textbf{11406.54} &  \textbf{11358.38} &  11314.18 \\
%           & halfcheetah-medium-v2 &            4996.88 &           5009.46 &            4989.70 &            4963.15 &           5006.02 &           3162.93 &   \textbf{5574.56} &   \textbf{5548.14} &   \textbf{5563.49} &   5544.29 \\
%           & hopper-expert-v2 &   \textbf{3592.58} &  \textbf{3534.48} &   \textbf{3601.80} &   \textbf{3598.00} &  \textbf{3438.49} &            577.40 &   \textbf{3321.27} &   \textbf{3255.01} &   \textbf{3153.23} &   3145.90 \\
%           & hopper-medium-v2 &   \textbf{1754.59} &           1649.30 &   \textbf{1732.90} &   \textbf{1742.17} &  \textbf{1878.75} &  \textbf{1869.26} &   \textbf{1827.40} &   \textbf{1998.11} &   \textbf{1844.06} &   1716.45 \\
%           & walker2d-expert-v2 &            4974.23 &           4966.13 &            4975.62 &            4994.30 &           4863.05 &            189.33 &   \textbf{5021.73} &   \textbf{5015.79} &   \textbf{5007.23} &   5006.99 \\
%           & walker2d-medium-v2 &            3269.71 &           3187.88 &   \textbf{3503.14} &            3321.13 &           3243.85 &           1345.95 &            3331.64 &            3377.36 &            3151.97 &   3473.84 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{table:raw_score_skewed}
% \end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}{lllll}
%     \toprule
%     {} & \multicolumn{2}{l}{BC} & \multicolumn{2}{l}{IQL} \\
%     {} &      Rw (0.1) & Uniform &      Aw (0.1) &      Rw (0.1) \\
%     Ratio &               &         &               &               \\
%     \midrule
%     1\%   &           0.7 &     0.4 &           2.2 &  \textbf{2.3} \\
%     5\%   &           2.8 &     0.2 &  \textbf{4.7} &           4.6 \\
%     10\%  &           3.0 &     0.2 &           3.1 &  \textbf{3.2} \\
%     50\%  &  \textbf{1.2} &     0.4 &           1.2 &           1.2 \\
%     100\% &           1.0 &     1.0 &  \textbf{1.0} &           1.0 \\
%     \bottomrule
%     \end{tabular}


%     \caption{Normalized median scores $(R_{algo} - R_{random}) / (R_{IQL (Uniform)}) - R_{Random}$}
%     \label{table:mujoco_perf}
% \end{table}

==> iclr2022/intro_backup.tex <==

\section{Introduction}
\label{sec:intro}

Offline reinforcement learning (RL) currently receives great attention because it allows to optimize RL policies from logged data without direct interaction with the environment. This makes the RL training process safer and cheaper since collecting interaction data is high-risk, expensive, and time-consuming in the real world (e.g., robotics, health care). Unfortunately, several papers showed that near optimality of the offline RL task is intractable sample-efficiency-wise. Indeed, \cite{Xiao2022} prove that passive data collection achieves a minimal number of state-action pair visits that decays exponentially either with the horizon or the number of states. Furthermore, 
%even if both concentrability and realizability are satisfied, 
any offline RL algorithm requires sample complexity either polynomial in the size of the state space or exponential in other parameters to learn a non-trivial policy~\citep{Chen2019,Foster2022}. These negative results advocate for another, tractable, objective.

In contrast to near optimality, policy improvement over the behavioral policy is an objective that is always approximately realizable since the behavioral policy may efficiently be cloned with supervised learning~\citep{Urbancic1994,Torabi2018}. Thus, most practical offline RL algorithms incorporate a component ensuring, either formally or intuitively, that the returned policy improves over the behavioral policy: pessimistic algorithms make sure that the target policy value's lower bound improves over the value of the behavioral policy~\citep{Petrik2016,kumar2020cql,buckman2020importance}, conservative algorithm regularize their policy search with respect to the behavioral policy~\citep{Thomas2015safe,Laroche2019,fujimoto2019off}, and one-step algorithms prevent the target policy value from propagating through bootstrapping~\citep{Brandfonbrener2021}. These algorithms use the behavioral policy as a stepping stone. As a consequence, their performance guarantees highly depend on the performance of the behavioral policy. To illustrate this dependency, we will say that these algorithms are anchored to the behavioral policy.
% Return-conditioned supervised learning (RCSL) is a notable exception~\citep{schmidhuber2019reinforcement, srivastava2019training,kumar2019reward,chen2021decision,furuta2021generalized}. RCSL consists in learning the return-conditional distribution of actions, and then sampling actions that receive high return. \cite{brandfonbrener2022does} prove that these methods are efficient under strong assumptions, including the determinism of the environment.

When an offline RL dataset consists in near-optimal trajectories, then the behavioral policy is itself near optimal, the anchoring is efficient, and the policy improvement opportunity is limited. When the dataset consists of low-performance trajectories, the behavioral policy is bad, the anchoring is neither helpful nor harmful, because the policy improvement opportunity is still limited: there is no good behavior to take inspiration from. Now, if a dataset is a mixture of low-performing and high-performing trajectories, the behavioral policy performance will be low to moderate, but the improvement opportunity high. This is the situation where the anchoring is detrimental to the potential policy improvement. We analyze that the potential for policy improvement over the behavioral policy is correlated with the positive-sided variance (PSV) of the trajectory returns in the dataset and advance that when the return PSV is high, the algorithmic anchoring may be limiting the performance of the returned policy.

In order to provide a better algorithmic anchor, we propose to alter the behavioral policy. We start by proving that reweighting the dataset during the training of an offline RL algorithm is equivalent to performing this training under another behavioral policy. Furthermore, under the assumption that the environment is deterministic, by giving larger weights to high-return trajectories, we can control the behavioral policy to be high performing and therefore grant a cold start performance boost to the offline RL algorithm. While determinism is a strong assumption that we prove to be necessary with a minimal failure example, we alleviate this limitation with the following observations. First, we note that determinism is also required for another popular class of offline RL algorithms: Return-conditioned supervised learning ~\citep[RCSL,][]{schmidhuber2019reinforcement,srivastava2019training,kumar2019reward,chen2021decision,furuta2021generalized,brandfonbrener2022does}. Second, we show that the guarantees still hold when the initial state is stochastic by reweighting with, instead of the trajectory return, a trajectory return advantage: $G(\tau_i)-V^\mu(s_{i,0})$, where $G(\tau_i)$ is the return obtained for trajectory $i$, $V^\mu(s_{i,0})$ is the expected return of following the behavioral policy $\mu$ from the initial state $s_{i,0}$. Third, we empirically observe that the strategy allows performance gains over their uniform sampling counterparts even in stochastic environments. 

% We further analyze that the positive-sided variance of the return distribution is a good predictor of the potential policy improvement over the behavioral policy, which existing Offline RL algorithms such as CQL, IQL, or TD3+BC fail to achieve. Indeed, mixed datasets of low-return and high-return trajectories have a low performing behavioral with therefore a high potential for improvement. Trajectory reweighting allows for significant boost in the induced behavioral policy performance, which provides a better anchor for the Offline RL algorithms.

% Experiments and their results here.
Under the guidance of theoretical analysis, our principal contribution is two simple weighted sampling strategies: \textbf{Return-weighted (RW)} and \textbf{Advantage-weighted (AW)} sampling. RW and AW re-weight trajectories using the Boltzmann distribution of trajectory returns and advantages, respectively. Our weighted sampling strategies are agnostic to the underlying offline RL algorithms and thus can be drop-in replacements for off-the-shelf offline RL algorithms. Moreover, the proposed sampling strategies do not incur extra computation during training. We evaluate our sampling strategies on three state-of-the-art offline RL algorithms~\citep{kumar2020cql,kostrikov2022offline,fujimoto2021minimalist} and behavior cloning over 62 datasets in D4RL benchmarks~\citep{fu2020d4rl}. The experimental results reported in statistically robust metrics~\citep{agarwal2021deep} display that both our sampling strategies significantly boost the performance of all offline RL algorithms in challenging mixed datasets with sparse rewarding trajectories and regular datasets with evenly distributed return distributions. Remarkably, our methods exhibit a statistically significant probability of improvements over the baselines.


==> iclr2022/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2022/problem_formulation_backup.tex <==
\section{Problem formulation}
\label{sec:psv_problem}
Most offline RL algorithms are anchored to the behavioral policy. This is beneficial when the dataset behavioral policy is high performing as it prevents them from overfitting on the data and degrade it. However, it can be detrimental when datasets are a mix of trajectories collected with low-performing novice policies and high-performing expert policies. Indeed, the anchoring restrains these algorithms from making sizable policy improvements over the behavioral policy of the mixed dataset, for which the performance is significantly lower than that of the expert policies. We formally define the return positive-sided variance (RPSV) of a dataset in Section~\ref{subsec:psv} and illustrate why the performance of offline RL algorithms could be limited on high-RPSV datasets in Section~\ref{subsec:issue_of_offlinerl}.

% We formulate the pitfall of offline RL in skewed datasets in this section. For example, a dataset consisting predominantly of episodes from a novice with a few episodes from an expert is a skewed dataset of particular interest. We formally define the skewness of a dataset in Section~\ref{subsec:skew} and illustrate why offline RL algorithms could fail on skewed datasets even when they have sufficient coverage of states and actions in Section~\ref{subsec:issue_of_offlinerl}.

% \begin{wrapfigure}{r}{0.5\textwidth}
% \vspace{-5ex}
%   \begin{center}
%     \includegraphics[width=0.5\textwidth]{iclr2022/figures/bernouli_plot.pdf}
%   \end{center}
%   \caption{Bernoulli distribution PSV: $\mathbb{V}_+[\mathcal{B}(p)]=p(1-p)^2$.}
% \vspace{-2ex}
%   \label{fig:bernoulli_psv}
% \end{wrapfigure}

\subsection{Positive-sided variance}
\label{subsec:psv}
% We need to define D and tau here
Formally, we are concerned with a dataset $\mathcal{D} := \{\tau_0, \tau_1, \cdots \tau_{N-1}\}$ potentially collected by various behavior policies $\{\mu_0, \mu_1,\cdots \mu_{N-1}\}$ and constituted of empirical returns $\{G(\tau_0), G(\tau_1), \cdots G(\tau_{N-1}) \}$, where $N$ is the number of trajectories, $T_i$ denotes the length of $\tau_i$, and $G(\tau_i) = \sum^{T_i-1}_{t=0}r_{i,t}$. To study the distribution of return, we equip ourselves with a statistical quantity: the positive-sided variance (PSV) of a random variable $X$:
\begin{definition}[Positive-sided variance]
\label{def:psv}
The positive-sided variance (PSV) of a random variable $X$ is the second-order moment of the positive component of $X-\mathbb{E}[X]$:
\begin{align}
    \mathbb{V}_{+}[X]&\doteq \mathbb{E}\left[\left(X-\mathbb{E}[X]\right)^2_{+}\right] \quad\text{with}\quad x_{+}=\max\{x,0\}.
\end{align}
\end{definition}
% \begin{definition}[Skewness]
% \label{def:skew}
% Let $N$ be the number of episodes in $\mathcal{D}$ and $\bar{G}(\mathcal{D}) = \frac{1}{N} \sum_{\tau_i \in\mathcal{D}} G(\tau_i)$. The skewness of a dataset $\mathcal{D}$, $\sk{\mathcal{D}}$,  is the third standardized moment, also known as the Fisher-Pearson coefficient of skewness~\citep{ziegel2001standard}, of the episodic returns $\{G(\tau_i) | \tau_i \in \mathcal{D}\}$:
% \begin{align}
%     \label{eq:skew}
%     \sk{\mathcal{D}} := \sk{\{G(\tau_i) | \tau_i \in \mathcal{D}\}} := \dfrac{1/N}{(1/N)^{3/2}} \dfrac{\sum^{N-1}_{i=0} (G(\tau_i) - \bar{G})^3}{(\sum^{N-1}_{i=0} (G(\tau_i) - \bar{G})^{2})^{3/2}}.
% \end{align}
% \end{definition}
We may symmetrically define the negative-sided variance $\mathbb{V}_-$ and notice that the variance is the sum of the two one-sided variances: $\mathbb{V}[X]=\mathbb{V}_{+}[X]+\mathbb{V}_{-}[X]$. The return PSV (RPSV) of $\mathcal{D}$ aims at capturing the positive dispersion of the distribution of the trajectory returns. An interesting question to ask is: \textit{what distribution leads to high RPSV?} We simplify sampling trajectories collected by a novice and an expert as sampling from a Bernoulli distribution $\mathcal{B}$, and suppose that the novice policy always yields a 0 return, while the expert always yields a 1 return. Figure~\ref{fig:bernoulli_psv} visualizes $\mathbb{V}_+[\mathcal{B}(p)]=p(1-p)^2$, which is the Bernoulli distribution's PSV as a function of its parameter $p$, where $p$ is the probability of choosing an expert trajectory. We see that maximal PSV is achieved for $p=\frac{1}{3}$ and both $p = 0$ (pure novice) and $p = 1$ (pure expert) leads to a zero PSV. This observation indicates that mixed datasets tend to have higher RPSV than a dataset collected by a single policy.  We present the return distribution of datasets at varying RPSV in Figure~\ref{fig:several_psv}. Low-RPSV dataset have their highest returns that remain close to the mean return, which limits the opportunity of policy improvement. In contrast, the return distribution of high-RPSV datasets disperse away from the mean toward the positive end. 
% It implies that the highest-PSV dataset is neither 
% \zwh{I feel it's unclear why we select Bernoulli to visualize. I think it's better to put a plot of real distribution of returns.}\romain{The idea is that Bernouilli emulates a mixing of two policies with deterministic returns. I do not have a strong opinion on which figure is better.} \zwh{Ah, good point. I like this argument. }\romain{We could even show what happens to this distribution after reweighting: $E[B(p)]=p \Rightarrow E[W_\alpha B(p)]=\frac{e^\alpha p}{e^\alpha p + 1-p}$}

\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.295\textwidth}
        \centering
        \includegraphics[width=\textwidth]{iclr2022/figures/bernouli_plot.pdf}
        \caption{Bernoulli distribution PSV}
        \label{fig:bernoulli_psv}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/psv_illustration_ant_medium-v2_0.01.pdf}
         \caption{Low RPSV}
         \label{fig:low_rpsv}
     \end{subfigure}
     \hfill
    %  \begin{subfigure}[b]{0.3\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figures/psv_illustration_ant_medium-v2_med.pdf}
    %      \caption{Moderate RPSV}
    %      \label{fig:med_rpsv}
    %  \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/psv_illustration_ant_medium-v2_0.5.pdf}
         \caption{High RPSV}
         \label{fig:high_rpsv}
     \end{subfigure}
     \caption{\textbf{(a)} Bernoulli distribution PSV: $\mathbb{V}_+[\mathcal{B}(p)]=p(1-p)^2$. \textbf{(b-c)} The return distribution of datasets with (b) low and (c) high return positive-sided variance (RPSV) (Section~\ref{subsec:psv}) , where RPSV measures the positive contributions in the variance of trajectory returns in a dataset and $\bar{G}$ denotes the average episodic returns (dashed line) of the dataset. Intuitively, a high RPSV implies some trajectories have far higher returns than the average.
    %  hence
    %  The high-PSV dataset consists primarily of low-return episodes and some high-return ones, and vice versa. A zero skewness indicates that returns are evenly distributed on both sides of the mean, instead of skewing towards either end. See Section~\ref{subsec:psv} for the details of $\sk{\mathcal{D}}$.
     }
     \label{fig:several_psv}
    %  \vspace{-4ex}
\end{figure}

==> iclr2022/zwh_intro.tex <==
Offline RL currently receives great attention since it allows to optimize RL policies from logged data without direct interaction with the environment. This makes the RL training process
